RNTuple: Towards First-Class Support for HPC data centers

Compared to LHC Run 1 and Run 2, future HEP experiments, e.g., at the HL-LHC, will increase the volume of generated data by an order of magnitude. In order to sustain the expected analysis throughput, ROOT's RNTuple I/O subsystem has been engineered to overcome the bottlenecks of the TTree I/O subsystem, focusing also on a compact data format, asynchronous and parallel requests, and a layered architecture that allows supporting distributed filesystem-less storage systems, e.g. HPC-oriented object stores. In a previous publication, we introduced and evaluated the RNTuple's native backend for Intel DAOS. Since its first prototype, we carried out a number of improvements both on RNTuple and its DAOS backend aiming to saturate the physical link, such as support for vector writes and an improved RNTuple-to-DAOS mapping, only to name a few. In parallel, the latest developments allow for better integration between RNTuple and ROOT's storage-agnostic, declarative interface to write HEP analyses, RDataFrame. In this work, we contribute with the following: (i) a redesign of the RNTuple DAOS backend, including a mechanism for efficient population of the object store based on existing data; and (ii) an experimental evaluation on a single-node platform, showing a significant increase in the analysis throughput for typical HEP workflows.

==> defs.tex <==
\def\RotHdr#1{\rlap{\rotatebox{45}{#1}}\rule{1.5em}{0pt}}
\def\Placeholder#1#2{\tikz\node[text width=\columnwidth,align=center,minimum height=#1,outer sep=4pt,draw]{--#2--};}
\def\TODO#1{\textcolor{red}{{\bf TODO:} #1}}


==> figs/daos-poolcontobj.tex <==
\tikz[container/.style 2 args={rounded corners,draw=#1!black!50,fill=#1!black!20,inner sep=4pt,label={above:#2}},
    every label/.style={font=\scriptsize},
    element/.style n args={3}{rounded corners,draw=#1!black!50,fill=#1!black!20,minimum width=#2,minimum height=#3,font=\fontsize{13}{13}\selectfont},
    target/.style 2 args={cylinder,shape border rotate=90,draw,right=1.75in of #1,inner sep=0pt,text width=20pt,minimum height=35pt,aspect=0.5,label={east:#2}},
    dkeyToTarget/.style={densely dashed,thick,draw=#1,->}
]{
    \def\zoomin#1#2{\draw[densely dashed,thick,black!50] (#1.north east) -- (#2.north west)
        (#1.south east) -- (#2.south west);}

    % Pool/containers
    \begin{scope}[start chain=c going below,node distance=4pt]
        \foreach \i in {1,2,3} \node[on chain,element={red!50}{1.5em}{1.5em}] {};
        \begin{pgfonlayer}{background}
            \node(P) [container={white!50}{DAOS pool},fit={(c-1)(c-3)}] {};
        \end{pgfonlayer}
    \end{scope}

    % Zoomed container
    \begin{scope}[start chain=o going below,node distance=4pt,xshift=1.5in]
        \foreach \i in {1,2,3} \node[on chain,element={olive!50}{2.3em}{1.3em}] {};
        \begin{pgfonlayer}{background}
            \node(C) [container={red!50}{DAOS container},fit={(o-1)(o-3)}] {};
        \end{pgfonlayer}
    \end{scope}
    \zoomin{c-2}{C}

    % Zoomed objects
    \begin{scope}[start chain=O going below,node distance=32pt,xshift=3.5in,yshift=1ex]
        \foreach \i in {1} \node[on chain,element={olive!50}{3.5em}{1.5em},inner ysep=1pt] {\color{olive!70!black!96}\begin{tabular}{|l|l|l|}\hline
        \texttt{dkey}    & \texttt{akey}    & \textit{value}     \\\hline
        \textcolor{red!60}{dkey1}  & \ldots & \ldots    \\\hline
        \end{tabular}};
        \foreach \i in {2} \node[on chain,element={olive!50}{3.5em}{2.80em},inner ysep=1pt] {\color{olive!70!black!96}\begin{tabular}{|l|l|l|}\hline
        \texttt{dkey}    & \texttt{akey}    & \textit{value}     \\\hline
        \textcolor{red!60}{dkey1}  & \ldots & \ldots    \\\hline
        \textcolor{blue!60}{dkey2}  & \ldots & \ldots    \\\hline
        \textcolor{red!60}{dkey1}  & \ldots & \ldots    \\\hline
        \end{tabular}};
        \node[above=0pt of O-1,font=\scriptsize] {DAOS object};
    \end{scope}
    \zoomin{o-1}{O-1}\zoomin{o-3}{O-2}

    \node(target1) [target={O-2}{Target 1},yshift=-20pt,xshift=-60pt]{};
    \node(target2) [target={O-2}{Target 2},yshift=25pt,xshift=-60pt]{};
    \node(targetDots) [above=5pt of target2]{\vdots};
    \node(targetN) [target={O-1}{Target $n$},yshift=5pt,xshift=-60pt]{};

    % FIXME: should use `\coordinate`s instead
    \draw[dkeyToTarget=red!60] ([yshift=7pt,xshift=-6pt]O-2.east) -- (target2);
    \draw[dkeyToTarget=red!60] ([yshift=-20pt,xshift=-6pt]O-2.east) -- (target2);
    \draw[dkeyToTarget=blue!60] ([yshift=-8pt,xshift=-6pt]O-2.east) -- (target1);
    \draw[dkeyToTarget=red!60] ([yshift=-8pt,xshift=-6pt]O-1.east) -- (targetN);

}   


==> figs/rntuple_daos_iovs.tex <==
\tikz[start chain=c going right,node distance=10pt,
      page/.style={minimum width=44pt,minimum height=24pt,inner xsep=34pt,inner ysep=2pt,
        draw=#1!76!black!76,fill=#1!76!black!20},
      iovs/.style={rectangle split,rectangle split parts=5,rectangle split horizontal,inner sep=10pt,
        draw,font={\bf\fontsize{25}{25}\selectfont},label={west:#1}},
      every label/.style={font={\fontsize{25}{25}\selectfont},text width=6in,align=center},
      >={Latex[length=1ex]},
]{
  \def\annotate#1#2#3#4{
    \draw[|-|] ([yshift=#1]#2.south west) -- ([yshift=#1]#3.south east) node [midway,above,font={\bfseries\fontsize{21}{31}\selectfont}] {#4};
  }

  % Pages
  \foreach \in [count=\c] in {1,2,...,5}
    \node(page-\c) [on chain=c,page=teal]{};
  \annotate{32pt}{page-1}{page-1}{Page 1}
  \annotate{32pt}{page-2}{page-2}{Page 2}
  \annotate{32pt}{page-5}{page-5}{Page $n$}
  \node [above=20pt of page-4]{\ldots};

  \node [draw,densely dashed,fit={(page-1)(page-5)},yshift=20pt,inner xsep=10pt,inner ysep=33pt]{};

  % IOVs
  \node (iovs)[iovs={Array of IOVs for a single akey},below=1.33in of page-1,anchor=west,xshift=-67pt]{%
    [0]
    \nodepart{two} [1]
    \nodepart{three} [2]
    \nodepart{four} \ldots\hspace{20pt}\ldots\hspace{20pt}\ldots
    \nodepart{five} [i]};

  \foreach \anchor/\p in {{text/page-1}, {two/page-2}, {five/page-5}}
    \draw[->] ([yshift=25pt]iovs.\anchor) -- (\p);
}


==> tweaks.tex <==
\setsansfont[BoldFont=FiraSans-Medium,ItalicFont=FiraSans-LightItalic]{FiraSans-Light}
\setmonofont[BoldFont=FiraCode-Medium]{FiraCode-Light}

\def\Large{\fontsize{32}{42}\selectfont}
\def\normalsize{\fontsize{26}{36}\selectfont}
\def\small{\fontsize{22}{32}\selectfont}
\def\tiny{\fontsize{20}{0}\selectfont}

\definecolor{alertfg}{HTML}{003049}
\setbeamercolor{caption name}{fg=black}
\setbeamertemplate{caption}{Fig.~\insertcaptionnumber: \insertcaption}
\setbeamercolor{alerted text}{fg=alertfg}

\setitemize{label=\raisebox{0.3ex}{\rule{0.7ex}{0.7ex}}}

\def\note#1{%
    \vspace{0.6em}
    \noindent #1
    \vspace{0.6em}
}

%\definecolor{heading1}{HTML}{023e8a}
%\definecolor{heading2}{HTML}{0077b6}
\definecolor{heading1}{HTML}{354f52}
\definecolor{heading2}{HTML}{52796f}
\definecolor{heading3}{HTML}{dee2e6}
\definecolor{heading4}{HTML}{f8f9fa}
\def\section#1{%
    \vspace{1ex}%
    \noindent\tikz\node[text width=\columnwidth,align=center,font={\Large\bfseries},white,
top color=heading1,bottom color=heading2,rounded corners=10,inner xsep=0pt]{#1};
    \setlength{\parindent}{1em}
}
\def\subsection#1{
    \vspace{1ex}%
    \noindent\tikz\node[text width=\columnwidth,align=center,font={\large\bfseries},black,
top color=heading3,bottom color=heading4,rounded corners=10,inner xsep=0pt]{#1};
}
\hypersetup{colorlinks=true,urlcolor=heading2,linkcolor=black}

\def\cite#1{\raisebox{0.5ex}{[#1]}}

